Optimal Communication and Control Strategies for a Multi-Agent System in the Presence of an Adversary

We consider a multi-agent system in which a decentralized team of agents controls a stochastic system in the presence of an adversary. Instead of committing to a fixed information sharing protocol, the agents can strategically decide at each time whether to share their private information with each other or not. The agents incur a cost whenever they communicate with each other and the adversary may eavesdrop on their communication. Thus, the agents in the team must effectively coordinate with each other while being robust to the adversary's malicious actions. We model this interaction between the team and the adversary as a stochastic zero-sum game where the team aims to minimize a cost while the adversary aims to maximize it. Under some assumptions on the adversary's capabilities, we characterize a min-max control and communication strategy for the team. We supplement this characterization with several structural results that can make the computation of the min-max strategy more tractable.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> constrained.tex <==
%Include constraints on 
%\bdashlist
%\item min and max time between successive comm
%\item total number of comms
%\end{list}
%in the problem formulation. 

In this section, we consider an extension of the problem formulated in Section \ref{sec:problem_formulation} where we incorporate some constraints on the communication between agents. The underlying system model,  information structure and the total expected cost  are the same as in Section \ref{sec:problem_formulation}. But now the agents have constraints on when and how frequently they can communicate. Specifically, we consider  the following three constraints:
\begin{enumerate}
\item Minimum time between successive communications must be at least $s_{min}$ (where $s_{min} \geq 0$).
\item Maximum time between successive communications cannot exceed $s_{max}$ (where $s_{max} \geq s_{min}$).
\item The total number of communications over the time horizon $T$ cannot exceed $N$.
\end{enumerate}
The strategy optimization problem is to find communication and control strategies for the agents that minimize the expected cost in \eqref{eq:cost2} while ensuring that the above three constraints are satisfied.  We assume that there is at least one choice of strategies for the agents for which the constraints are satisfied (i.e. the constrained problem is feasible). Note that our framework allows for some of the above three constraints to be absent (e.g. setting $s_{min}=0$ effectively removes the first constraint; setting $N=T$ effectively removes the third constraint). 

We can follow the methodology of Section \ref{Coordinator Results} for the constrained problem as well. The key difference is that in addition to the coordinator's beliefs on the agents' states, we will also need to keep track of (i) the time since the most recent communication (denoted by $S^a_t$), and (ii) the total number of  communications so far (denoted by $S^b_t$). The variables $S^a_t, S^b_t$ are used by the coordinator to make sure that the prescriptions it selects will not violate the constraints. For example, if $S^a_t < s_{min}$, the coordinator can only select the communication prescriptions  that map $\mathcal{X}^i$ to $0$ for each $i$ since this ensures that the first constraint will be satisfied. Similarly, if $S^a_t = s_{max}$, then the coordinator must select a pair of communication prescriptions that ensure that a communication happens at the current time. The following theorem describes the modified dynamic program for the coordinator in the constrained formulation.
\begin{theorem}
The value functions  for the coordinator's dynamic program are as follows: $V_{T+1}(\pi^1,\pi^2, s^a, s^b):=0$ for all $\pi^1,\pi^2, s^a,s^b,$ and for  $t=T, \ldots, 2, 1,$ \\
 \begin{align}
  &V_{t^+}(\pi^1,\pi^2, s^a, s^b) := \notag \\
 & \min_{\lambda^1, \lambda^2} \Big[\sum_{x^{1,2}}c_t\big(x^{1,2},\lambda^1(x^{1}),\lambda^2(x^{2})\big)\pi^1(x^1)\pi^2(x^2) \notag\\
 &+V_{t+1}(\beta_t( \pi^{1,2},\lambda^{1,2}),s^a,s^b)\Big],
\end{align}
where $\beta_t$ is as described in Lemma \ref{LEM:UPDATE}; and if $s_{min} \leq s^a < s_{max}$ and $s^b < N$
  \begin{align}
  &V_{t}(\pi^1,\pi^2,s^a,s^b) := \notag \\
 &\min_{\gamma^1, \gamma^2}\Big[\sum_{x^{1,2}}\rho(x^{1,2})\max(\gamma^1(x^{1}),\gamma^2(x^{2}))\pi^1(x^1)\pi^2(x^2) \notag \\ 
&+P(Z^{er}_t=\phi|\pi^{1,2},\gamma^{1,2}) V_{t^+}(\eta_t( \pi^{1,2},\gamma^{1,2}, \phi), s^a+1,s^b)\notag\\ &+\sum_{\tilde{x}^{1,2}}P(Z^{er}_t=\tilde{x}^{1,2}|\pi^{1,2},\gamma^{1,2})V_{t^+}(\delta_{\tilde{x}^1},\delta_{\tilde{x}^2},0,s^b+1)\Big], \label{eq:dp_gamma}
\end{align}
where $\eta_t$ is as described in Lemma \ref{LEM:UPDATE} and $P(Z^{er}_t=\phi|\pi^{1,2},\gamma^{1,2})$, $P(Z^{er}_t=\phi|\pi^{1,2},\gamma^{1,2})$ are as described by \eqref{eq:probz11} - \eqref{eq:probz22}. The coordinator's optimal strategy is to pick the minimizing prescription pairs for each time and each $(\pi^1,\pi^2)$.  If $s^b=N$ or if $s^a < s_{min}$, then the minimization over $\gamma^1,\gamma^2$ in \eqref{eq:dp_gamma} is replaced by simply setting $\gamma^1,\gamma^2$ to be the prescription that map all states to $0$. If $s^b < N$ and if $s^a = s_{max}$, then the minimization over $\gamma^1,\gamma^2$ in \eqref{eq:dp_gamma} is replaced by simply setting $\gamma^1,\gamma^2$ to be the prescription that map all states to $1$.   
\end{theorem}

%Write the corresponding pomdp dp.
%
%Can include the MDP version of the DP here.




==> erasure_state.tex <==
%Include constraints on 
%\bdashlist
%\item min and max time between successive comm
%\item total number of comms
%\end{list}
%in the problem formulation. 

In our formulation in Section \ref{sec:problem_formulation}, the quality of the erasure channel, i.e., the erasure probability $p_e$ did not change with time. In this section, we consider an extension of this formulation where the erasure probability evolves over time as an uncontrolled Markov process. Let $E_t \in \mathcal{E}$ denote the channel state at time $t$ where $\mathcal{E}$ is a finite set of channel states. The process $E_t$ evolves as $E_{t+1} = l_t(E_t,W_t^e)$ where the collection of variables $\{W_t^e\}_{t=1}^{\infty}$ is mutually independent and also independent of all the other primitive random variables. The erasure probability of the channel at time $t$ is a function of the channel state $E_t$, i.e., $p_{e_t} = \varphi_t(E_t)$. 

The channel state is known to both agents. The information available to agent $i$ at times $t$ (before communication) and $t^+$ (after communication) is thus given by 
\begin{align}
    I^i_{t}&=\{X^i_{1:t},U^i_{1:t-1},Z^{er}_{1:t-1},M^{1,2}_{1:t-1},E_{1:t}\}\\
    I^i_{t^+} &=\{I^i_{t},Z^{er}_t,M^{1,2}_t,E_{1:t}\}.
\end{align}
Our goal in this problem is to find communication and control strategies that minimize the total cost \eqref{eq:cost2} when the erasure channel quality is varying with time. With some minor modifications, we can use the common information based methodology of Section \ref{Coordinator Results} to solve this problem. 

If the coordinator's beliefs at time $t$ (before communication) are $\Pi^1_t, \Pi^2_t$, the channel state is $E_t$ and it selects the prescriptions $\Gamma^1_t, \Gamma^2_t,$ the probability that $Z^{er}_t=\phi$ (i.e. probability of no communication at time $t$) is given as 
% \begin{align}
% &P(Z_t=\phi|\Pi_t^{1,2},\Gamma_t^{1,2}) = \notag\\
%   &~~ =\sum_{x^1, x^2}\mathds{1}_{\{\Gamma^1_t(x^{1})=0\}}\mathds{1}_{\{\Gamma^2_t(x^{2})=0\}}\Pi^1_t(x^1)\Pi^2_t(x^2). \label{eq:probz1}
% \end{align}
\begin{align}
&P(Z^{er}_t=\phi|\Pi_t^{1,2},\Gamma_t^{1,2},E_t) = \notag\\
  &~~ =\sum_{x^1, x^2}\mathds{1}_{\{\Gamma^1(x^{1})=0\}}\mathds{1}_{\{\Gamma^2(x^{2})=0\}}\Pi^1_t(x^1)\Pi^2_t(x^2)\notag\\
  &+\sum_{x^1, x^2}\varphi_t(E_t)\Big[\max(\Gamma^1(x^{1}),\Gamma^2(x^{2}))\Big]\Pi^1_t(x^1)\Pi^2_t(x^2). \label{eq:probz11s}
\end{align}
Similarly, the probability that $Z^{er}_t = (x^1,x^2)$ is given as 
% \begin{align}
%     &P(Z_t=(x^1,x^2)|\Pi_t^{1,2},\Gamma_t^{1,2})\notag\\
%     &~~=\Big[\max(\Gamma^1_t(x^{1}),\Gamma^2_t(x^{2}))\Big]\Pi^1_t(x^1)\Pi^2_t(x^2). \label{eq:probz2}
%  \end{align}
\begin{align}
    &P(Z^{er}_t=(x^1,x^2)|\Pi_t^{1,2},\Gamma_t^{1,2})\notag\\
    &~~=(1-\varphi_t(E_t))\Big[\max(\Gamma^1(x^{1}),\Gamma^2(x^{2}))\Big]\Pi^1_t(x^1)\Pi^2_t(x^2). \label{eq:probz22s}
 \end{align}
The following theorem describes the modified dynamic program for the coordinator.
\begin{theorem}
The value functions  for the coordinator's dynamic program are as follows: $V_{T+1}(\pi^1,\pi^2, e):=0$ for all $\pi^1,\pi^2, e$, and for  $t=T, \ldots, 2, 1,$ \\
 \begin{align}
  &V_{t^+}(\pi^1,\pi^2, e) := \notag \\
 & \min_{\lambda^1, \lambda^2} \Big[\sum_{x^{1,2}}c_t\big(x^{1,2},\lambda^1(x^{1}),\lambda^2(x^{2})\big)\pi^1(x^1)\pi^2(x^2) \notag\\
 &+\E[V_{t+1}(\beta_t( \pi^{1,2},\lambda^{1,2}),E_{t+1})\mid E_t = e]\Big],
\end{align}
where $\beta_t$ is as described in Lemma \ref{LEM:UPDATE}, and
  \begin{align}
  &V_{t}(\pi^1,\pi^2,e) := \notag \\
 &\min_{\gamma^1, \gamma^2}\Big[\sum_{x^{1,2}}\rho(x^{1,2})\max(\gamma^1(x^{1}),\gamma^2(x^{2}))\pi^1(x^1)\pi^2(x^2) \notag \\ 
&+P(Z^{er}_t=\phi|\pi^{1,2},\gamma^{1,2},e) V_{t^+}(\eta_t( \pi^{1,2},\gamma^{1,2}, \phi), e)\notag\\ &+\sum_{\tilde{x}^{1,2}}P(Z^{er}_t=\tilde{x}^{1,2}|\pi^{1,2},\gamma^{1,2},e)V_{t^+}(\delta_{\tilde{x}^1},\delta_{\tilde{x}^2},e)\Big], \label{eq:dp_gamma}
\end{align}
where $\eta_t$ is as described in Lemma \ref{LEM:UPDATE} and $P(Z^{er}_t=\phi|\pi^{1,2},\gamma^{1,2},e)$, $P(Z^{er}_t=\phi|\pi^{1,2},\gamma^{1,2},e)$ are as described by \eqref{eq:probz11s} - \eqref{eq:probz22s}. The coordinator's optimal strategy is to pick the minimizing prescription pairs for each time and each $(\pi^1,\pi^2)$.
\end{theorem}




%Write the corresponding pomdp dp.
%
%Can include the MDP version of the DP here.




==> experiments.tex <==
\textbf{Problem setup} Consider a system where there are two entities that are susceptible to attacks. Each entity has an associated defender that can either choose to do nothing (denoted by $\aleph$) or defend the system. The defender has access to two defensive actions $d_1$ and $d_2$. Thus, the defenders are the decision-making agents in this model. The state $X_t^i \in \{0,1\}$ of agent $i$ represents whether or not entity $i$ is under attack at time $t$. We use 1 to denote the \emph{attack} state and 0 to denote the \emph{safe} (non-attack) state.  If entity $i$ is currently in the safe state, i.e. $X^i_t = 0$, then with probability $p^i_a$, the entity transitions to the attack state 1 (irrespective of the defender's action). When entity $i$ is under attack, i.e. $X_t^i = 1$, if the corresponding defender chooses to do nothing, then the state does not change with probability 1, i.e. $X_{t+1}^i = X_t^{i}$. On the other hand, if the defender chooses to defend using defensive action $d_k$ where $k=1,2$, then the entity transitions to the safe state 0 with probability $p^i_{d_k}$ and thus, vanquishing the attacker. The transition probabilities can found in a tabular form in Table \ref{trans}.  If both entities are in the safe state, then the cost incurred by the system is 0. If at least one entity is under attack, then the cost incurred is 20. Further, an additional cost of 100 (150 resp.) is incurred if both defenders choose to defend using $d_1$ (resp. $d_2$) at the same time (in any state). More explicitly,
\begin{align*}
c_t(X_t,U_t) = \vartheta^{t-1}\big[20\mathds{1}_{(X_t^1 = 1 \text{ or } X_t^2 = 1)} &+ 100\mathds{1}_{(U_t^1 = d^1)}\mathds{1}_{(U_t^2 = d^1)}\\
& + 150\mathds{1}_{(U_t^1 = d^2)}\mathds{1}_{(U_t^2 = d^2)}\big],
\end{align*}
where $0<\vartheta\leq 1$ is a discount factor.

When an entity is under attack, the associated defender needs to defend the system at some point of time (if not immediately). Otherwise, the system will remain in the attack state perpetually. However, a heavy cost is incurred if both agents defend using the same defensive action. Therefore, the agents must defend their respective entities in a coordinated manner. Communicating with each other can help in coordinating effectively. On the other hand, communicating all the time can also lead to a high communication cost. This tradeoff between communication and coordination can be balanced optimally using our approach discussed in Section \ref{Coordinator Results}.

%Our model shares some similarities with the multi-access broadcast problem with limited buffers. Note that unlike in \cite{hansen2004dynamic}, the transmitters in our model can choose to communicate with each other before using the broadcast channel.

\begin{table}[t]
\caption{Transition probabilities $\prob[X^i_{t+1} \mid X^i_t, U^i_t]$.}
\label{trans}
\vskip -0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccr}
\toprule
 & $U_t^i = \aleph$ & $U_t^i = d_1$ & $U_t^i = d_2$ \\
\midrule
$X_t^i = 0$   & (1-$p^i_a$,$p_a^i$)& (1-$p^i_a$,$p_a^i$)&  (1-$p^i_a$,$p_a^i$)\\
$X_t^i = 1$   & (0,1)& ($p^i_{d_1}$,1-$p_{d_1}^i$)& ($p^i_{d_2}$,1-$p_{d_2}^i$)\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%
%
%\begin{table}[t]
%\caption{The cost $c_t(X_t,U_t) = \vartheta^{t-1}c(x,u)$ where $\vartheta$ is the discount factor and the function $c(x,u)$ is shown below. Each row corresponds to a pair of actions $u := (u^{1},u^{2})$ and each column corresponds to a state $x:=(x^1,x^2)$.}
%\label{costable}
%%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccccr}
%\toprule
% & $(0,0)$ & $(0,1)$ & $(1,0)$ & $(1,1)$ \\
%\midrule
%$(\aleph, \aleph)$   & 0 & 20& 20& 20\\
%$(\aleph,d)$   & 0& 20& 20 & 20\\
%$(d,\aleph)$   & 0& 20& 20 & 20\\
%$(d,d)$   & 150 & 170& 170& 170\\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}

\textbf{Implementation} In our experiments, the transition probabilities are time invariant and the cost is discounted. The time horizon infinite. We use an infinite-horizon POMDP solver to find approximately optimal finite horizon cost for the coordinator's POMDP. Since the agents alternate between communication and control (see equations \eqref{commact1} and \eqref{controlact1}), the coordinator's POMDP as described in  Section \ref{Coordinator Results} is not time-invariant. To convert it into a time-invariant POMDP, we introduce an additional binary state variable $X_t^{c}$. This variable represents whether the agents currently are in the communication phase or the control phase. The variable $X_t^c$ alternates between 0 and 1 in a deterministic manner. For agent $i$ in the communication phase, action $\aleph$ is interpreted as the no communication decision ($M_t^i = 0$) and all other actions (in this case only $d$) are interpreted as the communication decision ($M_t^i = 1$).




With this transformation, we can use any infinite-horizon POMDP solver to obtain approximately optimal solutions for our problem. In our experiments, we use the SARSOP solver \cite{kurniawati2008sarsop} that is available in the Julia POMDPs framework \cite{egorov2017pomdps}.


%\begin{remark}
%As discussed in Remark \ref{infiniteremark}, the procedure described above can be used to find optimal values and strategies even for the case when the time-horizon is infinite.
%\end{remark}



\textbf{Results} We consider three strategies in our experiments: (i) the jointly optimal communication and control strategy computed using the coordinator's POMDP, (ii) agents never communicate with each other and the control strategy is optimized subject to this constraint, and (iii) agents always communicate with each other and the control strategy is optimized subject to this constraint. The expected cost associated with these three strategies is shown in Figure \ref{fig1}. The approximation error achieved using the SARSOP solver is at most 0.001.

\textbf{Scaling up} {A major challenge in solving the coordinator's POMDP is that the prescription space is exponential in state size $\mathcal{X}^i$. Recall that in the coordinator's POMDP, the coordinator's action space is the joint prescription space. POMDP solvers need to optimize over the POMDP's action space (in this case prescription space) repeatedly as an intermediate step \cite{kurniawati2008sarsop}. A naive approach for optimizing over the prescription space is to enumerate every prescription and choose the one with the optimum value. This approach is commonly used because the action space in POMDPs is fairly small.  In \cite{dibangoye2012scaling,dibangoye2013producing} an approach based on constraint optimization \cite{dechter2003constraint} was proposed to tackle the computational complexity involved in the exhaustive enumeration of all the prescriptions. It was noted in \cite{dibangoye2012scaling,dibangoye2013producing} that this approach works significantly better in practice. Our current implementation based on the Julia framework can be used only when the prescription space is small. In order to solve larger scale problems, one can modify the algorithm in \cite{kurniawati2008sarsop} to incorporate the constraint optimization approach in \cite{dibangoye2012scaling,dibangoye2013producing}.
%When state spaces are large, even single stage problems are very difficult to solve. In such situations, one can use alternative approaches as in \cite{foerster2019bayesian} wherein the prescriptions are parameterized in a concise manner. However, these methods are not guaranteed to result in optimal solutions.
}


\begin{figure}
\centering
\includegraphics[width = \columnwidth]{fig_strat.eps}
\caption{Performance achieved by three strategies: jointly optimal communication and coordination protocol, (ii) always communicate, and (iii) never communicate. In this example, $p^1_a = p^2_a = 0.3$, $p^1_{d_1} = p^2_{d_1} = 0.6$, $p^1_{d_2} = p^2_{d_2} = 0.4$ and $\vartheta = 0.95$.}
\label{fig1}
\end{figure}
%\begin{table}[t]
%\caption{Optimal costs with initial state $X_1 = (0,0)$ under different communication strategies. The parameters $p^i_a = 0.3$ and $p^i_v = 0.6$, $i = 1,2$. The discount factor $\vartheta$ is $0.95$.}
%\label{res1}
%%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccccr}
%\toprule
% & Optimal & Never comm. & Always comm. \\
%\midrule
%$\rho = 0$   & 105.86 & 120.42& 105.86\\
%$\rho = 1$   & 108.45 & 120.42& 116.12\\
%$\rho = 2$   & 111.05 & 120.42& 126.37\\
%$\rho = 4$   & 116.24 & 120.42& 146.89\\
%$\rho = 8$   & 120.42 & 120.42& 187.96\\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}
%
%\begin{table}[t]
%\caption{Optimal costs with initial state $X_1 = (0,0)$ under different communication strategies. The parameters $p^1_a = 0.5$, $p^1_v = 0.95$, $p_a^2 = 0.1$ and $p_v^2 = 0.6$. The discount factor $\vartheta$ in this case is $0.99$.}
%\label{res2}
%%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccccr}
%\toprule
% & Optimal & Never comm. & Always comm. \\
%\midrule
%$\rho = 0$   & 452.18 & 538.13& 452.87\\
%$\rho = 1$   & 459.05 & 538.13& 502.43\\
%$\rho = 2$   & 465.93 & 538.13& 552.68\\
%$\rho = 4$   & 479.64 & 538.13& 653.19\\
%$\rho = 8$   & 504.26 & 538.13& 854.19\\
%$\rho = 16$   & 537.86 & 538.13& 1256.21\\
%$\rho = 32$   & 538.13 & 538.13& 2060.23\\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}




